Binding Dancers Into Attractors

To effectively perceive and process observations in our environment, feature binding and perspective taking are crucial cognitive abilities. Feature binding combines observed features into one entity, called a Gestalt. Perspective taking transfers the percept into a canonical, observer-centered frame of reference. Here we propose a recurrent neural network model that solves both challenges. We first train an LSTM to predict 3D motion dynamics from a canonical perspective. We then present similar motion dynamics with novel viewpoints and feature arrangements. Retrospective inference enables the deduction of the canonical perspective. Combined with a robust mutual-exclusive softmax selection scheme, random feature arrangements are reordered and precisely bound into known Gestalt percepts. To corroborate evidence for the architecture's cognitive validity, we examine its behavior on the silhouette illusion, which elicits two competitive Gestalt interpretations of a rotating dancer. Our system flexibly binds the information of the rotating figure into the alternative attractors resolving the illusion's ambiguity and imagining the respective depth interpretation and the corresponding direction of rotation. We finally discuss the potential universality of the proposed mechanisms.

==> dancer-sequence/dancer-postures.tikz.tex <==
\begin{scope}[xshift=0.0cm, yshift=0.0]
\node[posture_point_style] (p0) at (0.01821243, 0.052314743) {};
\node[posture_point_style] (p1) at (-0.018412247, 0.047100335) {};
\node[posture_point_style] (p2) at (0.0026935115, -0.03950584) {};
\node[posture_point_style] (p3) at (0.04257511, 0.052314743) {};
\node[posture_point_style] (p4) at (0.03805197, -0.024744779) {};
\node[posture_point_style] (p5) at (0.026688945, -0.13015029) {};
\node[posture_point_style] (p6) at (0.03039377, 0.09553942) {};
\node[posture_point_style] (p7) at (0.03039377, 0.14305715) {};
\node[posture_point_style] (p8) at (0.03039377, 0.19823968) {};
\node[posture_point_style] (p9) at (0.0048633274, 0.16520861) {};
\node[posture_point_style] (p10) at (0.024096256, 0.21764669) {};
\node[posture_point_style,left_hand_style] (p11) at (0.048829988, 0.23289788) {};
\node[posture_point_style] (p12) at (0.058675595, 0.1476247) {};
\node[posture_point_style] (p13) at (0.111641906, 0.09806821) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\node[posture_point_style,right_hand_style] (p14) at (0.11797122, 0.08618878) {};
\end{scope}
\begin{scope}[xshift=1.1cm, yshift=0.0]
\node[posture_point_style] (p0) at (-0.08501741, -0.020378947) {};
\node[posture_point_style] (p1) at (-0.30469224, -0.035799824) {};
\node[posture_point_style] (p2) at (-0.11174619, -0.2919257) {};
\node[posture_point_style] (p3) at (0.016704012, -0.02037894) {};
\node[posture_point_style] (p4) at (-0.06093757, -0.24827182) {};
\node[posture_point_style] (p5) at (-0.09081912, -0.55999404) {};
\node[posture_point_style] (p6) at (-0.034156702, 0.107452095) {};
\node[posture_point_style] (p7) at (-0.034156702, 0.24797928) {};
\node[posture_point_style] (p8) at (-0.034156702, 0.41117403) {};
\node[posture_point_style] (p9) at (-0.12282366, 0.31348905) {};
\node[posture_point_style] (p10) at (-0.17290574, 0.46856752) {};
\node[posture_point_style,left_hand_style] (p11) at (-0.14981553, 0.5136707) {};
\node[posture_point_style] (p12) at (0.060756914, 0.26148707) {};
\node[posture_point_style] (p13) at (-0.024470806, 0.11493066) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07086846, 0.07979886) {};
\end{scope}
\begin{scope}[xshift=2.2cm, yshift=0.0]
\node[posture_point_style] (p0) at (0.09760628, -0.09516656) {};
\node[posture_point_style] (p1) at (0.48370108, -0.120864995) {};
\node[posture_point_style] (p2) at (0.16293898, -0.54808766) {};
\node[posture_point_style] (p3) at (-0.09364262, -0.095166095) {};
\node[posture_point_style] (p4) at (0.028685402, -0.47518772) {};
\node[posture_point_style] (p5) at (0.09176278, -0.99459547) {};
\node[posture_point_style] (p6) at (0.001887556, 0.11978085) {};
\node[posture_point_style] (p7) at (0.0018563268, 0.35466605) {};
\node[posture_point_style] (p8) at (0.0018383018, 0.62685484) {};
\node[posture_point_style] (p9) at (0.1757787, 0.46417767) {};
\node[posture_point_style] (p10) at (0.21758963, 0.7226732) {};
\node[posture_point_style,left_hand_style] (p11) at (0.14206879, 0.7977962) {};
\node[posture_point_style] (p12) at (-0.1858056, 0.3772335) {};
\node[posture_point_style] (p13) at (-0.14814857, 0.13288972) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.09000473, 0.07453587) {};
\end{scope}
\begin{scope}[xshift=3.3000000000000003cm, yshift=0.0]
\node[posture_point_style] (p0) at (0.06579779, -0.098734215) {};
\node[posture_point_style] (p1) at (0.37159526, -0.12465589) {};
\node[posture_point_style] (p2) at (0.08298646, -0.5588848) {};
\node[posture_point_style] (p3) at (-0.06256853, -0.0986728) {};
\node[posture_point_style] (p4) at (0.06057197, -0.48472172) {};
\node[posture_point_style] (p5) at (0.09053908, -1.0122653) {};
\node[posture_point_style] (p6) at (0.0014624002, 0.12022953) {};
\node[posture_point_style] (p7) at (0.0014728804, 0.3590728) {};
\node[posture_point_style] (p8) at (0.0014413609, 0.63586307) {};
\node[posture_point_style] (p9) at (0.105731525, 0.47053778) {};
\node[posture_point_style] (p10) at (0.22487816, 0.73324656) {};
\node[posture_point_style,left_hand_style] (p11) at (0.23021117, 0.8096401) {};
\node[posture_point_style] (p12) at (-0.10828887, 0.38205802) {};
\node[posture_point_style] (p13) at (0.13133879, 0.13390873) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\node[posture_point_style,right_hand_style] (p14) at (0.2193138, 0.07527792) {};
\end{scope}
\begin{scope}[xshift=4.4cm, yshift=0.0]
\node[posture_point_style] (p0) at (0.0015756246, -0.09979578) {};
\node[posture_point_style] (p1) at (0.0772648, -0.1262135) {};
\node[posture_point_style] (p2) at (-0.03885139, -0.56400263) {};
\node[posture_point_style] (p3) at (-0.00026658765, -0.099974245) {};
\node[posture_point_style] (p4) at (0.06421656, -0.48925015) {};
\node[posture_point_style] (p5) at (0.045821503, -1.021334) {};
\node[posture_point_style] (p6) at (0.00060814933, 0.1203902) {};
\node[posture_point_style] (p7) at (0.00061811326, 0.36109638) {};
\node[posture_point_style] (p8) at (0.0006035919, 0.6402497) {};
\node[posture_point_style] (p9) at (-0.016968053, 0.47344464) {};
\node[posture_point_style] (p10) at (0.12387968, 0.7383593) {};
\node[posture_point_style,left_hand_style] (p11) at (0.20950621, 0.8154086) {};
\node[posture_point_style] (p12) at (0.023794062, 0.3842643) {};
\node[posture_point_style] (p13) at (0.35444185, 0.13401473) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\node[posture_point_style,right_hand_style] (p14) at (0.43252632, 0.07517616) {};
\end{scope}
\begin{scope}[xshift=5.5cm, yshift=0.0]
\node[posture_point_style] (p0) at (-0.06342794, -0.09973568) {};
\node[posture_point_style] (p1) at (-0.25673315, -0.12682976) {};
\node[posture_point_style] (p2) at (-0.14296648, -0.56641257) {};
\node[posture_point_style] (p3) at (0.06362176, -0.09977669) {};
\node[posture_point_style] (p4) at (0.03793845, -0.4913567) {};
\node[posture_point_style] (p5) at (-0.020666786, -1.0263109) {};
\node[posture_point_style] (p6) at (0.000116561736, 0.120421134) {};
\node[posture_point_style] (p7) at (0.00012472848, 0.3620668) {};
\node[posture_point_style] (p8) at (0.00011381771, 0.6424376) {};
\node[posture_point_style] (p9) at (-0.13236001, 0.4748016) {};
\node[posture_point_style] (p10) at (-0.036741987, 0.74098057) {};
\node[posture_point_style,left_hand_style] (p11) at (0.08931337, 0.8183756) {};
\node[posture_point_style] (p12) at (0.14677632, 0.38531122) {};
\node[posture_point_style] (p13) at (0.4119117, 0.13380115) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\node[posture_point_style,right_hand_style] (p14) at (0.442095, 0.074081704) {};
\end{scope}
\begin{scope}[xshift=6.6000000000000005cm, yshift=0.0]
\node[posture_point_style] (p0) at (-0.09831004, -0.09989766) {};
\node[posture_point_style] (p1) at (-0.4705273, -0.12690088) {};
\node[posture_point_style] (p2) at (-0.17954281, -0.56750405) {};
\node[posture_point_style] (p3) at (0.098182626, -0.0998475) {};
\node[posture_point_style] (p4) at (-0.0060658543, -0.49230555) {};
\node[posture_point_style] (p5) at (-0.07740784, -1.0286032) {};
\node[posture_point_style] (p6) at (-4.4227454e-05, 0.12046499) {};
\node[posture_point_style] (p7) at (-4.2089432e-05, 0.36251757) {};
\node[posture_point_style] (p8) at (-4.675867e-05, 0.6434818) {};
\node[posture_point_style] (p9) at (-0.18527928, 0.4754107) {};
\node[posture_point_style] (p10) at (-0.18052173, 0.7422583) {};
\node[posture_point_style,left_hand_style] (p11) at (-0.073539324, 0.81983364) {};
\node[posture_point_style] (p12) at (0.20131713, 0.38579628) {};
\node[posture_point_style] (p13) at (0.27502614, 0.13361435) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\node[posture_point_style,right_hand_style] (p14) at (0.24195556, 0.07346607) {};
\end{scope}
\begin{scope}[xshift=7.700000000000001cm, yshift=0.0]
\node[posture_point_style] (p0) at (-0.06187104, -0.078494176) {};
\node[posture_point_style] (p1) at (-0.117129475, -0.35583997) {};
\node[posture_point_style] (p2) at (-0.072973624, -0.34662572) {};
\node[posture_point_style] (p3) at (-0.04194414, -0.0886805) {};
\node[posture_point_style] (p4) at (-0.07292163, -0.35383624) {};
\node[posture_point_style] (p5) at (-0.06736679, -0.3580872) {};
\node[posture_point_style] (p6) at (-0.05825945, 0.11354288) {};
\node[posture_point_style] (p7) at (-0.07102884, 0.34617218) {};
\node[posture_point_style] (p8) at (-0.07401992, 0.32736498) {};
\node[posture_point_style] (p9) at (-0.09121349, 0.39487323) {};
\node[posture_point_style] (p10) at (-0.110502124, 0.38579446) {};
\node[posture_point_style,left_hand_style] (p11) at (-0.107451014, 0.40110865) {};
\node[posture_point_style] (p12) at (-0.07494362, 0.38197353) {};
\node[posture_point_style] (p13) at (-0.15932277, 0.39023846) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.1821981, 0.37646675) {};
\end{scope}
\begin{scope}[xshift=8.8cm, yshift=0.0]
\node[posture_point_style] (p0) at (0.05564598, -0.100404754) {};
\node[posture_point_style] (p1) at (0.09317654, -0.3382756) {};
\node[posture_point_style] (p2) at (0.079191625, -0.6596171) {};
\node[posture_point_style] (p3) at (-0.059749015, -0.087139525) {};
\node[posture_point_style] (p4) at (0.056543864, -0.22630672) {};
\node[posture_point_style] (p5) at (0.0708443, -0.6482314) {};
\node[posture_point_style] (p6) at (-0.0071533816, 0.11569989) {};
\node[posture_point_style] (p7) at (-0.0096323, 0.3312034) {};
\node[posture_point_style] (p8) at (0.0022851825, 0.6167515) {};
\node[posture_point_style] (p9) at (0.04500302, 0.38636294) {};
\node[posture_point_style] (p10) at (-0.0091272835, 0.43373996) {};
\node[posture_point_style,left_hand_style] (p11) at (-0.035960607, 0.3902012) {};
\node[posture_point_style] (p12) at (-0.053333685, 0.43102622) {};
\node[posture_point_style] (p13) at (0.0075623803, 0.48463544) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.011822057, 0.496065) {};
\end{scope}
\begin{scope}[xshift=9.9cm, yshift=0.0]
\node[posture_point_style] (p0) at (0.067013144, -0.09973048) {};
\node[posture_point_style] (p1) at (0.026326459, -0.48024967) {};
\node[posture_point_style] (p2) at (-0.027039874, -0.9981075) {};
\node[posture_point_style] (p3) at (-0.055379104, -0.10007744) {};
\node[posture_point_style] (p4) at (-0.25800294, -0.14414532) {};
\node[posture_point_style] (p5) at (-0.13967213, -0.5483388) {};
\node[posture_point_style] (p6) at (0.0011287639, 0.11939022) {};
\node[posture_point_style] (p7) at (0.0041109417, 0.35340938) {};
\node[posture_point_style] (p8) at (0.0035324031, 0.6348894) {};
\node[posture_point_style] (p9) at (0.13890906, 0.37929827) {};
\node[posture_point_style] (p10) at (0.3370751, 0.13871586) {};
\node[posture_point_style,left_hand_style] (p11) at (0.38516486, 0.112878405) {};
\node[posture_point_style] (p12) at (-0.11705035, 0.4507579) {};
\node[posture_point_style] (p13) at (-0.035661995, 0.74283105) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\node[posture_point_style,right_hand_style] (p14) at (0.07182586, 0.77527726) {};
\end{scope}
\begin{scope}[xshift=11.0cm, yshift=0.0]
\node[posture_point_style] (p0) at (0.09772112, -0.100733966) {};
\node[posture_point_style] (p1) at (-0.012361641, -0.48517302) {};
\node[posture_point_style] (p2) at (-0.08086569, -1.0099394) {};
\node[posture_point_style] (p3) at (-0.09759436, -0.09756316) {};
\node[posture_point_style] (p4) at (-0.46809483, -0.12937386) {};
\node[posture_point_style] (p5) at (-0.17551395, -0.5722723) {};
\node[posture_point_style] (p6) at (5.6352234e-05, 0.11977945) {};
\node[posture_point_style] (p7) at (-0.00025695364, 0.35940823) {};
\node[posture_point_style] (p8) at (-0.00611602, 0.6389566) {};
\node[posture_point_style] (p9) at (0.19353437, 0.38420838) {};
\node[posture_point_style] (p10) at (0.24478579, 0.14553313) {};
\node[posture_point_style,left_hand_style] (p11) at (0.21049966, 0.0850693) {};
\node[posture_point_style] (p12) at (-0.17749672, 0.47302797) {};
\node[posture_point_style] (p13) at (-0.18104309, 0.7321596) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.07983626, 0.79865175) {};
\end{scope}
\begin{scope}[xshift=12.100000000000001cm, yshift=0.0]
\node[posture_point_style] (p0) at (0.08345113, -0.10034265) {};
\node[posture_point_style] (p1) at (-0.050055813, -0.48947918) {};
\node[posture_point_style] (p2) at (-0.098118015, -1.0223736) {};
\node[posture_point_style] (p3) at (-0.08444539, -0.10091404) {};
\node[posture_point_style] (p4) at (-0.4518253, -0.12867972) {};
\node[posture_point_style] (p5) at (-0.1246976, -0.5675346) {};
\node[posture_point_style] (p6) at (-0.0002492726, 0.11995614) {};
\node[posture_point_style] (p7) at (-0.0008095539, 0.36224183) {};
\node[posture_point_style] (p8) at (-0.002696939, 0.64296657) {};
\node[posture_point_style] (p9) at (0.1519279, 0.38538712) {};
\node[posture_point_style] (p10) at (-0.010042292, 0.13855971) {};
\node[posture_point_style,left_hand_style] (p11) at (-0.08280061, 0.07773585) {};
\node[posture_point_style] (p12) at (-0.14440313, 0.47379202) {};
\node[posture_point_style] (p13) at (-0.23652112, 0.736716) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.20564914, 0.81348974) {};
\end{scope}
\begin{scope}[xshift=13.200000000000001cm, yshift=0.0]
\node[posture_point_style] (p0) at (0.029902138, -0.09990125) {};
\node[posture_point_style] (p1) at (-0.066396564, -0.4917006) {};
\node[posture_point_style] (p2) at (-0.06888148, -1.02664) {};
\node[posture_point_style] (p3) at (-0.030518297, -0.099946275) {};
\node[posture_point_style] (p4) at (-0.21791776, -0.12770179) {};
\node[posture_point_style] (p5) at (-0.014108294, -0.5685034) {};
\node[posture_point_style] (p6) at (-0.00017673356, 0.12007032) {};
\node[posture_point_style] (p7) at (-0.0003800378, 0.36368474) {};
\node[posture_point_style] (p8) at (-0.0016793924, 0.64339983) {};
\node[posture_point_style] (p9) at (0.035813846, 0.38711378) {};
\node[posture_point_style] (p10) at (-0.27477905, 0.13564056) {};
\node[posture_point_style,left_hand_style] (p11) at (-0.36413836, 0.07485191) {};
\node[posture_point_style] (p12) at (-0.037921745, 0.4744519) {};
\node[posture_point_style] (p13) at (-0.17814276, 0.7404699) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.23222487, 0.8167412) {};
\end{scope}
\begin{scope}[xshift=14.3cm, yshift=0.0]
\node[posture_point_style] (p0) at (-0.038220547, -0.0999585) {};
\node[posture_point_style] (p1) at (-0.052152064, -0.49245855) {};
\node[posture_point_style] (p2) at (-0.007958799, -1.0291343) {};
\node[posture_point_style] (p3) at (0.03788925, -0.100506306) {};
\node[posture_point_style] (p4) at (0.12073101, -0.12751728) {};
\node[posture_point_style] (p5) at (0.10456328, -0.567512) {};
\node[posture_point_style] (p6) at (-7.377074e-05, 0.12030516) {};
\node[posture_point_style] (p7) at (-0.00013977749, 0.36190537) {};
\node[posture_point_style] (p8) at (-0.00072698935, 0.64443624) {};
\node[posture_point_style] (p9) at (-0.09929582, 0.38629222) {};
\node[posture_point_style] (p10) at (-0.41188625, 0.13480859) {};
\node[posture_point_style,left_hand_style] (p11) at (-0.46771714, 0.07392606) {};
\node[posture_point_style] (p12) at (0.08796899, 0.47577745) {};
\node[posture_point_style] (p13) at (-0.034352258, 0.7423319) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\node[posture_point_style,right_hand_style] (p14) at (-0.14966604, 0.8186927) {};
\end{scope}


==> dancer-sequence/posturestyles.tikz.tex <==
\definecolor{posture_link_color}{RGB}{0, 0, 0}
%\definecolor{posture_pos_color}{RGB}{224, 169, 90}

\definecolor{posture_pos_color}{RGB}{150, 150, 150}
%\definecolor{posture_vel_color}{RGB}{50, 129, 194}

\definecolor{posture_vel_color}{RGB}{130, 200, 70}
\definecolor{syscolor}{RGB}{240,213,199}
\definecolor{contextcolor}{RGB}{172,92,0}
%\definecolor{optboxcolor}{RGB}{250,250,250}
%\definecolor{backpresentcolor}{RGB}{70,130,180}
%\definecolor{backpastcolor}{RGB}{70,130,180}
%\definecolor{backoptcolor}{RGB}{220,100,20}
\definecolor{boxcolorback}{RGB}{186,208,206}
\definecolor{bindingvalue}{RGB}{70,130,180}


\def\nnpointwidth{0.5cm}

\tikzstyle{posture_point_style} = [circle,fill=posture_pos_color,draw=posture_link_color,minimum width=0.08cm, inner sep=0]

\tikzstyle{posture_link_style} = [draw=posture_link_color,thick]

\tikzstyle{posture_vel_style} = [draw=posture_vel_color,semithick,round cap-round cap]


\tikzstyle{posture_pos_box_style} = [
    draw=posture_pos_color!50!black,rounded corners=0.1cm,inner sep=0,minimum height=0.6cm,minimum width=0.8cm,
    top color = posture_pos_color!5!white,
    bottom color = posture_pos_color!20!white,
    nnstyleshadow
]

\tikzstyle{posture_vel_box_style} = [
    draw=posture_vel_color!50!black,rounded corners=0.1cm,inner sep=0,minimum   height=0.6cm,minimum width=0.8cm,
    top color = posture_vel_color!5!white,
    bottom color = posture_vel_color!10!white,
    nnstyleshadow
]


\tikzstyle{modulestyle} = [
    rectangle,
    rounded corners=0.1cm,
    top color = incellcolor!10!white,
    bottom color = incellcolor!40!white,
    draw =  incellcolor!60!black,
    minimum width=\nnopwidth,
    minimum height=\nnopheight,
    inner sep=0
]

\tikzstyle{left_hand_style} = [
    draw=blue!50!black,fill=blue
]

\tikzstyle{right_hand_style} = [
    draw=red!50!black,fill=red
]

\tikzstyle{righthand_style} = [
    draw=posture_vel_color!50!black,rounded corners=0.1cm,inner sep=0,minimum   height=0.6cm,minimum width=0.8cm,
    top color = posture_vel_color!5!white,
    bottom color = posture_vel_color!10!white,
    nnstyleshadow
]


\definecolor{gflowcolor}{RGB}{152,54,59}


==> dancer-sequence/tikzlibraryneural.code.tex <==
\usepackage{upgreek}

\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows.meta}


\usetikzlibrary{positioning}

\usetikzlibrary{shadows}
\usetikzlibrary{shadows.blur}



% ----------------------------------------------------------------
% distance definitions.
% ----------------------------------------------------------------
\def\nncellwidth{0.5cm}
\def\nncellhwidth{0.25cm}
\def\nnsmallcellwidth{0.3cm}
\def\nntinycellwidth{0.2cm}

\def\nnshadowoffset{0.075cm}


% ----------------------------------------------------------------
% cell and node styles.
% ----------------------------------------------------------------
\tikzstyle{nnstylecell} = [circle,fill=white,draw=black,minimum width=\nncellwidth, inner sep=0]

\tikzstyle{nnstylesmallcell} = [circle,fill=white,draw=black,minimum width=\nnsmallcellwidth, inner sep=0]

\tikzstyle{nnstyletinycell}  = [circle,fill=white,draw=black,minimum width=\nntinycellwidth, inner sep=0]


% ----------------------------------------------------------------
% link styles.
% ----------------------------------------------------------------
\tikzstyle{nnstyleline}    = [draw=black]      
\tikzstyle{nnstylelink}    = [draw=black,-latex]
\tikzstyle{nnstylelinkbid} = [draw=black,latex-latex]


% ----------------------------------------------------------------
% other styles.
% ----------------------------------------------------------------
\tikzstyle{nndashed} = [dash pattern=on 2pt off 1.0pt]


%
% name, at, width, height, content
%
\newcommand{\nnbox}[5]{
    \node[rectangle,fill=white!90!black,minimum width=#3, minimum height=#4, inner sep=0] at ($(\nnshadowoffset,-\nnshadowoffset)+(#2)$) {};\node[rectangle,fill=white,draw=black,minimum width=#3, minimum height=#4, inner sep=0] (#1) at (#2) {#5};
}

\newcommand{\nnboxback}[5]{
    \node[rectangle,fill=black, opacity=0.1, minimum width=#3, minimum height=#4, inner sep=0] at ($(\nnshadowoffset,-\nnshadowoffset)+(#2)$) {};\node[rectangle,fill=white,draw=black,minimum width=#3, minimum height=#4, inner sep=0] (#1) at (#2) {#5};
}


\newcommand{\nnboxspec}[6]{%
    \node[rectangle,fill=white!90!black,minimum width=#3, minimum height=#4, inner sep=0] at ($(\nnshadowoffset,-\nnshadowoffset)+(#2)$) {};\node[rectangle,fill=white,draw=black,minimum width=#3, minimum height=#4, inner sep=0,#6] (#1) at (#2) {#5};
}




% ----------------------------------------------------------------
% predifined cell types.
% ----------------------------------------------------------------
\newcommand*{\nnnonlinear}[2]{
    
    \node[nnstylecell] (#1) at (#2) {};
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
        \draw[black] (#1_p1) edge[distance=\nncellhwidth,out=0,in=180] (#1_p2);
        %\draw[black] ($(#1.south west)+(0.01,0.002)$) edge[out=0,in=180] ($(#1.north east)-(0.01,0.002)$);
    }
}

\newcommand*{\nnspacercell}[2]{
    \node[nnstylecell,fill=none,draw=none] (#1) at (#2) {};
}

\newcommand*{\nndashedcell}[2]{
    \node[nnstylecell,nndashed,draw=gray] (#1) at (#2) {};
}

\newcommand*{\nndashedsmallcell}[2]{
    \node[nnstylesmallcell,nndashed, draw=gray,fill=none] (#1) at (#2) {};
}

\newcommand*{\nndashedtinycell}[2]{
    \node[nnstyletinycell,nndashed, draw=gray,fill=none] (#1) at (#2) {};
}

\newcommand*{\nnlabelcell}[3]{
    \node[nnstylecell] (#1) at (#2) {#3}; % \sum
}


\newcommand*{\nnlinear}[2]{
    \node[nnstylecell] (#1) at (#2) {$$};
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
        \draw[black] (#1_p1) -- (#1_p2);
    }
}

\newcommand*{\nncell}[2]{
    \node[nnstylecell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
    }
}

\newcommand*{\nnsmallcell}[2]{
    \node[nnstylesmallcell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
    }
}

\newcommand*{\nnsmallcellarg}[3]{
    \node[nnstylesmallcell, #3] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
    }
}


\newcommand*{\nntinycell}[2]{
    \node[nnstyletinycell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
    }
}

% ----------------------------------------------------------------
% other stuff.
% ----------------------------------------------------------------


%
% name, at, width, height, content
%


%
% name, at, width, height, bordercolor, backgroundcolor, content
%
\newcommand{\nnboxnoshad}[7]{%
    \node[rectangle,fill=#6,draw=#5,minimum width=#3, minimum height=#4, outer sep = 0,inner sep=0,rounded corners=0.05cm] (#1) at (#2) {#7};
}

















\newcommand*{\cellspacer}[2]{
    \node[style_cell,fill=none,draw=none] (#1) at (#2) {};
}

\newcommand*{\cellfollow}[2]{
    \node[style_cell,dashed,draw=gray] (#1) at (#2) {};
}

\newcommand*{\colorcell}[3]{
    \node[style_smallcell,fill=#3] (#1) at (#2) {};
}

\newcommand*{\valueinput}[3]{
    \node[style_cell] (#1) at (#2) {#3}; % \sum
}

\newcommand*{\inlinks}[3]{
    \draw[style_link,#3] ($(#1.center)+({#2-30}:1.1cm)$) -- (#1);
    \node[rotate=#2-90,#3] at ($(#1.center)+({#2}:0.7cm)$) {\small{$\cdots$}};
    \draw[style_link,#3] ($(#1.center)+({#2+30}:1.1cm)$) -- (#1);
}

\newcommand*{\outlinks}[3]{
    \draw[style_link,#3] (#1) -- ($(#1.center)+({#2-30}:0.8cm)$);
    \node[rotate=#2-90,#3] at ($(#1.center)+({#2}:0.5cm)$) {\small{$\cdots$}};
    \draw[style_link,#3] (#1) -- ($(#1.center)+({#2+30}:0.8cm)$);
}
\newcommand*{\oldlinear}[2]{
    \node[style_cell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\hcellwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\hcellwidth)$);
        \draw[black] (#1_p1) -- (#1_p2);
        %\draw[black] ($(#1.south west)+(0.01,0.01)$) -- ($(#1.north east)-(0.01,0.01)$);
    }
}

\newcommand*{\oldcell}[2]{
    \node[style_cell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\hcellwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\hcellwidth)$);
        %\draw[black] ($(#1.south west)+(0.01,0.01)$) -- ($(#1.north east)-(0.01,0.01)$);
    }
}

\newcommand*{\mult}[2]{
    \node[style_smallcell] (#1) at (#2) {$\Uppi$};
}

\newcommand*{\dmult}[2]{
    \node[style_smallcell] (#1) at (#2) {\small{$\partial \Pi$}};
}

\newcommand*{\con}[2]{
    \node[style_con] (#1) at (#2) {};
}

\newcommand*{\convar}[3]{
    \node[style_con,#3] (#1) at (#2) {};
}





\def\boxWidth{5cm}
\def\boxHeight{3cm}

\def\nncellwidth{0.5cm}
\def\nncellhwidth{0.25cm}
\def\nnsmallcellwidth{0.35cm}
\def\nntinycellwidth{0.15cm}

\def\nnopwidth{0.65cm}
\def\nnopheight{0.35cm}


\definecolor{boxcolorback}{RGB}{186,208,206}
\definecolor{cellcolor}{RGB}{208,160, 160}
\definecolor{incellcolor}{RGB}{186,208,206}

\tikzstyle{nnstylesmallcell} = [
circle,
top color = cellcolor!30!white,
bottom color = cellcolor!50!white,
draw =  cellcolor!40!black,
minimum width=\nnsmallcellwidth,
inner sep=0]


\tikzstyle{nnstyleop} = [
rectangle,
rounded corners=0.1cm,
top color = cellcolor!20!white,
bottom color = cellcolor!50!white,
draw =  cellcolor!40!black,
minimum width=\nnopwidth,
minimum height=\nnopheight,
inner sep=0]

\tikzstyle{nnstyleinop} = [
rectangle,
rounded corners=0.1cm,
top color = incellcolor!20!white,
bottom color = incellcolor!50!white,
draw =  cellcolor!40!black,
minimum width=\nnopwidth,
minimum height=\nnopheight,
inner sep=0]


\tikzstyle{nnstylelink} = [
draw=black!80!white,
rounded corners = 0.1cm,
-Kite,
]

\tikzstyle{nnstyleline} = [
draw=cellcolor!20!black,
rounded corners = 0.1cm
]

\tikzstyle{nnstylebox} = [
rectangle,
rounded corners=0.1cm,
top color = incellcolor!20!white,
bottom color = incellcolor!50!white,
draw =  cellcolor!40!black,
minimum width=\nnopwidth,
minimum height=\nnopheight,
inner sep=0
]


\tikzstyle{nnstyleboxdark} = [
rectangle,
top color = boxcolorback!70!white,
bottom color = boxcolorback!80!black,
draw=boxcolorback!40!black,
outer sep = 0,
inner sep=0,
rounded corners=0.1cm
]


\tikzstyle{nnstyleshadow} = [
blur shadow = {%
    shadow yshift=-0.5pt,
    shadow xshift=0.5pt,
    shadow blur radius=1pt,
    shadow blur extra rounding,
    shadow blur steps=5,
    shadow scale=0.99,
    shadow opacity=50
}
]


==> model/posture-first.tikz.tex <==
\begin{scope}[xshift=0.0, yshift=0.0]
\node[posture_point_style] (p0) at (0.15839391028356947, -0.20556353) {};
\node[posture_point_style] (p1) at (-0.007396468716348983, -0.98761136) {};
\node[posture_point_style] (p2) at (-0.4211782042636822, -1.82454348) {};
\node[posture_point_style] (p3) at (0.022361753483077715, -0.2061781) {};
\node[posture_point_style] (p4) at (0.3827362180046166, -0.91226136) {};
\node[posture_point_style] (p5) at (0.6117143829453107, -1.83312928) {};
\node[posture_point_style] (p6) at (0.017057396639556778, 0.237589732) {};
\node[posture_point_style] (p7) at (0.05946770801121567, 0.7083016) {};
\node[posture_point_style] (p8) at (0.0715958372483623, 1.2515058) {};
\node[posture_point_style] (p9) at (0.20342617515424355, 0.884732) {};
\node[posture_point_style] (p10) at (0.5263719308320174, 0.051306106) {};
\node[posture_point_style] (p11) at (0.6887249820940741, -0.128565952) {};
\node[posture_point_style] (p12) at (-0.16821057999442596, 0.87829114) {};
\node[posture_point_style] (p13) at (-0.14219147332782134, -0.06362688) {};
\node[posture_point_style] (p14) at (-0.11872177002477535, -0.3067488) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\draw[posture_vel_style] (p0.center) --++ (-0.00213954501773229, -0.005005896);
\draw[posture_vel_style] (p1.center) --++ (0.17630449658706848, -0.04960656);
\draw[posture_vel_style] (p2.center) --++ (-0.2060361023267323, 0.02693832);
\draw[posture_vel_style] (p3.center) --++ (-0.004773286855184266, 0.0057846309);
\draw[posture_vel_style] (p4.center) --++ (-0.04389048459298881, -0.0241604448);
\draw[posture_vel_style] (p5.center) --++ (-0.22320480962433228, -0.068228244);
\draw[posture_vel_style] (p6.center) --++ (-0.010346487990260606, 0.0008922815400000001);
\draw[posture_vel_style] (p7.center) --++ (-0.01712944444098775, 0.0027287007);
\draw[posture_vel_style] (p8.center) --++ (-0.011597247875465736, 0.0055915116);
\draw[posture_vel_style] (p9.center) --++ (-0.025460246927186066, -0.0040465593);
\draw[posture_vel_style] (p10.center) --++ (-0.10827956433390012, -0.043843389);
\draw[posture_vel_style] (p11.center) --++ (-0.12670690587878572, -0.067658274);
\draw[posture_vel_style] (p12.center) --++ (-0.009680078223946361, 0.0082978605);
\draw[posture_vel_style] (p13.center) --++ (0.027318990885339407, 0.00146470965);
\draw[posture_vel_style] (p14.center) --++ (0.015837722714970897, -0.0031104683999999996);
\end{scope}


==> model/posture-second.tikz.tex <==
\begin{scope}[xshift=0.0, yshift=0.0]
\node[posture_point_style] (p0) at (0.15466758789563775, -0.21226896) {};
\node[posture_point_style] (p1) at (0.17401595988369736, -1.0127104) {};
\node[posture_point_style] (p2) at (-0.4384040305916839, -1.77402008) {};
\node[posture_point_style] (p3) at (0.01742035842706814, -0.19717133) {};
\node[posture_point_style] (p4) at (0.315078635129741, -0.94217604) {};
\node[posture_point_style] (p5) at (0.45508588592949484, -1.8743154) {};
\node[posture_point_style] (p6) at (0.018375612429165154, 0.23752454) {};
\node[posture_point_style] (p7) at (0.060536213496221875, 0.70861864) {};
\node[posture_point_style] (p8) at (0.06243905873989223, 1.2523135) {};
\node[posture_point_style] (p9) at (0.19495672878193696, 0.87985664) {};
\node[posture_point_style] (p10) at (0.4589930408498455, 0.022540454) {};
\node[posture_point_style] (p11) at (0.6037936784827149, -0.17325438) {};
\node[posture_point_style] (p12) at (-0.16060869040404488, 0.8822565) {};
\node[posture_point_style] (p13) at (-0.12900160739982758, -0.05671047) {};
\node[posture_point_style] (p14) at (-0.09824598411153723, -0.2970926) {};
\draw[posture_link_style] (p0) -- (p1);
\draw[posture_link_style] (p1) -- (p2);
\draw[posture_link_style] (p3) -- (p4);
\draw[posture_link_style] (p4) -- (p5);
\draw[posture_link_style] (p6) -- (p0);
\draw[posture_link_style] (p6) -- (p3);
\draw[posture_link_style] (p7) -- (p6);
\draw[posture_link_style] (p8) -- (p7);
\draw[posture_link_style] (p7) -- (p9);
\draw[posture_link_style] (p9) -- (p10);
\draw[posture_link_style] (p10) -- (p11);
\draw[posture_link_style] (p7) -- (p12);
\draw[posture_link_style] (p12) -- (p13);
\draw[posture_link_style] (p13) -- (p14);
\draw[posture_vel_style] (p0.center) --++ (0.0002337822683251423, -0.00354409218);
\draw[posture_vel_style] (p1.center) --++ (0.29949021017840566, 0.0038409234);
\draw[posture_vel_style] (p2.center) --++ (0.2224380445736611, 0.12260377500000001);
\draw[posture_vel_style] (p3.center) --++ (-0.013474641058912521, 0.0031790883);
\draw[posture_vel_style] (p4.center) --++ (-0.1031927477890602, -0.042848289);
\draw[posture_vel_style] (p5.center) --++ (-0.22693606853232678, -0.028722882);
\draw[posture_vel_style] (p6.center) --++ (0.009517401849516487, -0.0007550418300000001);
\draw[posture_vel_style] (p7.center) --++ (0.022009016104124927, -0.0012552738000000002);
\draw[posture_vel_style] (p8.center) --++ (0.007619087000639747, -0.0028806924);
\draw[posture_vel_style] (p9.center) --++ (0.001006172730936077, -0.0145268439);
\draw[posture_vel_style] (p10.center) --++ (-0.09451482707915346, -0.061564689);
\draw[posture_vel_style] (p11.center) --++ (-0.10053170913900784, -0.086742639);
\draw[posture_vel_style] (p12.center) --++ (0.04184909206782605, 0.010322033999999999);
\draw[posture_vel_style] (p13.center) --++ (0.09692426209559765, 0.022686235500000002);
\draw[posture_vel_style] (p14.center) --++ (0.13863821929948209, 0.02875194);
\end{scope}


==> model/posturestyles.tikz.tex <==
\definecolor{posture_link_color}{RGB}{0, 0, 0}
%\definecolor{posture_pos_color}{RGB}{224, 169, 90}

\definecolor{posture_pos_color}{RGB}{150, 150, 150}
%\definecolor{posture_vel_color}{RGB}{50, 129, 194}

\definecolor{posture_vel_color}{RGB}{130, 200, 70}
\definecolor{syscolor}{RGB}{240,213,199}
\definecolor{contextcolor}{RGB}{172,92,0}
%\definecolor{optboxcolor}{RGB}{250,250,250}
%\definecolor{backpresentcolor}{RGB}{70,130,180}
%\definecolor{backpastcolor}{RGB}{70,130,180}
%\definecolor{backoptcolor}{RGB}{220,100,20}
\definecolor{boxcolorback}{RGB}{186,208,206}
\definecolor{bindingvalue}{RGB}{70,130,180}


\def\nnpointwidth{0.5cm}

\tikzstyle{posture_point_style} = [circle,fill=posture_pos_color,draw=posture_link_color,minimum width=0.12cm, inner sep=0]

\tikzstyle{posture_link_style} = [draw=posture_link_color,thick]

\tikzstyle{posture_vel_style} = [draw=posture_vel_color,semithick,round cap-round cap]


\tikzstyle{posture_pos_box_style} = [
    draw=posture_pos_color!50!black,rounded corners=0.1cm,inner sep=0,minimum height=0.6cm,minimum width=0.8cm,
    top color = posture_pos_color!5!white,
    bottom color = posture_pos_color!20!white,
    nnstyleshadow
]

\tikzstyle{posture_vel_box_style} = [
    draw=posture_vel_color!50!black,rounded corners=0.1cm,inner sep=0,minimum   height=0.6cm,minimum width=0.8cm,
    top color = posture_vel_color!5!white,
    bottom color = posture_vel_color!10!white,
    nnstyleshadow
]


\tikzstyle{modulestyle} = [
    rectangle,
    rounded corners=0.1cm,
    top color = incellcolor!10!white,
    bottom color = incellcolor!40!white,
    draw =  incellcolor!60!black,
    minimum width=\nnopwidth,
    minimum height=\nnopheight,
    inner sep=0
]


\definecolor{gflowcolor}{RGB}{152,54,59}


==> model/tikzlibraryneural.code.tex <==
\usepackage{upgreek}

\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows.meta}


\usetikzlibrary{positioning}

\usetikzlibrary{shadows}
\usetikzlibrary{shadows.blur}



% ----------------------------------------------------------------
% distance definitions.
% ----------------------------------------------------------------
\def\nncellwidth{0.5cm}
\def\nncellhwidth{0.25cm}
\def\nnsmallcellwidth{0.3cm}
\def\nntinycellwidth{0.2cm}

\def\nnshadowoffset{0.075cm}


% ----------------------------------------------------------------
% cell and node styles.
% ----------------------------------------------------------------
\tikzstyle{nnstylecell} = [circle,fill=white,draw=black,minimum width=\nncellwidth, inner sep=0]

\tikzstyle{nnstylesmallcell} = [circle,fill=white,draw=black,minimum width=\nnsmallcellwidth, inner sep=0]

\tikzstyle{nnstyletinycell}  = [circle,fill=white,draw=black,minimum width=\nntinycellwidth, inner sep=0]


% ----------------------------------------------------------------
% link styles.
% ----------------------------------------------------------------
\tikzstyle{nnstyleline}    = [draw=black]      
\tikzstyle{nnstylelink}    = [draw=black,-latex]
\tikzstyle{nnstylelinkbid} = [draw=black,latex-latex]


% ----------------------------------------------------------------
% other styles.
% ----------------------------------------------------------------
\tikzstyle{nndashed} = [dash pattern=on 2pt off 1.0pt]


%
% name, at, width, height, content
%
\newcommand{\nnbox}[5]{
    \node[rectangle,fill=white!90!black,minimum width=#3, minimum height=#4, inner sep=0] at ($(\nnshadowoffset,-\nnshadowoffset)+(#2)$) {};\node[rectangle,fill=white,draw=black,minimum width=#3, minimum height=#4, inner sep=0] (#1) at (#2) {#5};
}

\newcommand{\nnboxback}[5]{
    \node[rectangle,fill=black, opacity=0.1, minimum width=#3, minimum height=#4, inner sep=0] at ($(\nnshadowoffset,-\nnshadowoffset)+(#2)$) {};\node[rectangle,fill=white,draw=black,minimum width=#3, minimum height=#4, inner sep=0] (#1) at (#2) {#5};
}


\newcommand{\nnboxspec}[6]{%
    \node[rectangle,fill=white!90!black,minimum width=#3, minimum height=#4, inner sep=0] at ($(\nnshadowoffset,-\nnshadowoffset)+(#2)$) {};\node[rectangle,fill=white,draw=black,minimum width=#3, minimum height=#4, inner sep=0,#6] (#1) at (#2) {#5};
}




% ----------------------------------------------------------------
% predifined cell types.
% ----------------------------------------------------------------
\newcommand*{\nnnonlinear}[2]{
    
    \node[nnstylecell] (#1) at (#2) {};
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
        \draw[black] (#1_p1) edge[distance=\nncellhwidth,out=0,in=180] (#1_p2);
        %\draw[black] ($(#1.south west)+(0.01,0.002)$) edge[out=0,in=180] ($(#1.north east)-(0.01,0.002)$);
    }
}

\newcommand*{\nnspacercell}[2]{
    \node[nnstylecell,fill=none,draw=none] (#1) at (#2) {};
}

\newcommand*{\nndashedcell}[2]{
    \node[nnstylecell,nndashed,draw=gray] (#1) at (#2) {};
}

\newcommand*{\nndashedsmallcell}[2]{
    \node[nnstylesmallcell,nndashed, draw=gray,fill=none] (#1) at (#2) {};
}

\newcommand*{\nndashedtinycell}[2]{
    \node[nnstyletinycell,nndashed, draw=gray,fill=none] (#1) at (#2) {};
}

\newcommand*{\nnlabelcell}[3]{
    \node[nnstylecell] (#1) at (#2) {#3}; % \sum
}


\newcommand*{\nnlinear}[2]{
    \node[nnstylecell] (#1) at (#2) {$$};
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
        \draw[black] (#1_p1) -- (#1_p2);
    }
}

\newcommand*{\nncell}[2]{
    \node[nnstylecell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
    }
}

\newcommand*{\nnsmallcell}[2]{
    \node[nnstylesmallcell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
    }
}

\newcommand*{\nnsmallcellarg}[3]{
    \node[nnstylesmallcell, #3] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
    }
}


\newcommand*{\nntinycell}[2]{
    \node[nnstyletinycell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\nncellhwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\nncellhwidth)$);
    }
}

% ----------------------------------------------------------------
% other stuff.
% ----------------------------------------------------------------


%
% name, at, width, height, content
%


%
% name, at, width, height, bordercolor, backgroundcolor, content
%
\newcommand{\nnboxnoshad}[7]{%
    \node[rectangle,fill=#6,draw=#5,minimum width=#3, minimum height=#4, outer sep = 0,inner sep=0,rounded corners=0.05cm] (#1) at (#2) {#7};
}

















\newcommand*{\cellspacer}[2]{
    \node[style_cell,fill=none,draw=none] (#1) at (#2) {};
}

\newcommand*{\cellfollow}[2]{
    \node[style_cell,dashed,draw=gray] (#1) at (#2) {};
}

\newcommand*{\colorcell}[3]{
    \node[style_smallcell,fill=#3] (#1) at (#2) {};
}

\newcommand*{\valueinput}[3]{
    \node[style_cell] (#1) at (#2) {#3}; % \sum
}

\newcommand*{\inlinks}[3]{
    \draw[style_link,#3] ($(#1.center)+({#2-30}:1.1cm)$) -- (#1);
    \node[rotate=#2-90,#3] at ($(#1.center)+({#2}:0.7cm)$) {\small{$\cdots$}};
    \draw[style_link,#3] ($(#1.center)+({#2+30}:1.1cm)$) -- (#1);
}

\newcommand*{\outlinks}[3]{
    \draw[style_link,#3] (#1) -- ($(#1.center)+({#2-30}:0.8cm)$);
    \node[rotate=#2-90,#3] at ($(#1.center)+({#2}:0.5cm)$) {\small{$\cdots$}};
    \draw[style_link,#3] (#1) -- ($(#1.center)+({#2+30}:0.8cm)$);
}
\newcommand*{\oldlinear}[2]{
    \node[style_cell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\hcellwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\hcellwidth)$);
        \draw[black] (#1_p1) -- (#1_p2);
        %\draw[black] ($(#1.south west)+(0.01,0.01)$) -- ($(#1.north east)-(0.01,0.01)$);
    }
}

\newcommand*{\oldcell}[2]{
    \node[style_cell] (#1) at (#2) {$$}; % \sum
    {
        \coordinate (#1_p1) at ($(#2) - (45:\hcellwidth)$);
        \coordinate (#1_p2) at ($(#2) + (45:\hcellwidth)$);
        %\draw[black] ($(#1.south west)+(0.01,0.01)$) -- ($(#1.north east)-(0.01,0.01)$);
    }
}

\newcommand*{\mult}[2]{
    \node[style_smallcell] (#1) at (#2) {$\Uppi$};
}

\newcommand*{\dmult}[2]{
    \node[style_smallcell] (#1) at (#2) {\small{$\partial \Pi$}};
}

\newcommand*{\con}[2]{
    \node[style_con] (#1) at (#2) {};
}

\newcommand*{\convar}[3]{
    \node[style_con,#3] (#1) at (#2) {};
}





\def\boxWidth{5cm}
\def\boxHeight{3cm}

\def\nncellwidth{0.5cm}
\def\nncellhwidth{0.25cm}
\def\nnsmallcellwidth{0.35cm}
\def\nntinycellwidth{0.15cm}

\def\nnopwidth{0.65cm}
\def\nnopheight{0.35cm}


\definecolor{boxcolorback}{RGB}{186,208,206}
\definecolor{cellcolor}{RGB}{208,160, 160}
\definecolor{incellcolor}{RGB}{186,208,206}

\tikzstyle{nnstylesmallcell} = [
circle,
top color = cellcolor!30!white,
bottom color = cellcolor!50!white,
draw =  cellcolor!40!black,
minimum width=\nnsmallcellwidth,
inner sep=0]


\tikzstyle{nnstyleop} = [
rectangle,
rounded corners=0.1cm,
top color = cellcolor!20!white,
bottom color = cellcolor!50!white,
draw =  cellcolor!40!black,
minimum width=\nnopwidth,
minimum height=\nnopheight,
inner sep=0]

\tikzstyle{nnstyleinop} = [
rectangle,
rounded corners=0.1cm,
top color = incellcolor!20!white,
bottom color = incellcolor!50!white,
draw =  cellcolor!40!black,
minimum width=\nnopwidth,
minimum height=\nnopheight,
inner sep=0]


\tikzstyle{nnstylelink} = [
draw=black!80!white,
rounded corners = 0.1cm,
-Kite,
]

\tikzstyle{nnstyleline} = [
draw=cellcolor!20!black,
rounded corners = 0.1cm
]

\tikzstyle{nnstylebox} = [
rectangle,
rounded corners=0.1cm,
top color = incellcolor!20!white,
bottom color = incellcolor!50!white,
draw =  cellcolor!40!black,
minimum width=\nnopwidth,
minimum height=\nnopheight,
inner sep=0
]


\tikzstyle{nnstyleboxdark} = [
rectangle,
top color = boxcolorback!70!white,
bottom color = boxcolorback!80!black,
draw=boxcolorback!40!black,
outer sep = 0,
inner sep=0,
rounded corners=0.1cm
]


\tikzstyle{nnstyleshadow} = [
blur shadow = {%
    shadow yshift=-0.5pt,
    shadow xshift=0.5pt,
    shadow blur radius=1pt,
    shadow blur extra rounding,
    shadow blur steps=5,
    shadow scale=0.99,
    shadow opacity=50
}
]

